Deployment and configuration of MEC apps with Simu5G

Multi-access Edge Computing (MEC) is expected to act as the enabler for the integration of 5G (and future 6G) communication technologies with cloud-computing-based capabilities at the edge of the network. This will enable low-latency and context-aware applications for users of such mobile networks. In this paper we describe the implementation of a MEC model for the Simu5G simulator and illustrate how to configure the environment to evaluate MEC applications in both simulation and real-time emulation modes.

==> OMNeT++ Community Summit 2021 - Simu5G_MEC/temptex <==
\begin{lstlisting}
{
    "appDid" : "WAMECAPP",
    "appName" : "MECWarningAlertApp",
    "appProvider" : "lte.apps.mec.warningAlert.MECWarningAlertApp",
    "virtualComputeDescriptor" :{
        "virtualDisk": 10,
        "virtualCpu" : 1500,
        "virtualMemory":10
    },
    "appServiceRequired": [{
        "ServiceDependency" :{
            "serName" : "LocationService",
            "version" : "v2",
            "serCategory": "Location"
        }
    }
    ]
}
\end{lstlisting}


\begin{lstlisting}
#------------UEWarningAlertApp---------------
*.car[*].numApps = 2

# .car[*].app[0] is the DeviceApp
*.car[*].app[0].typename = "DeviceApp"
*.car[*].app[0].localPort = 4500
*.car[*].app[0].lcmProxyAddress = "lcmProxy"
*.car[*].app[0].lcmProxyPort = 1000

*.car[*].app[1].typename = "UEWarningAlertApp"
# Device App address
*.car[*].app[1].destAddress = "car["+string(ancestorIndex(1))+"]"   
# Device App port
*.car[*].app[1].destPort = 4500   
\end{lstlisting}





\begin{lstlisting}
    ######################_MEC Hosts Side_#####################
    # available resources 
    *.meHost*.maxMEApps = 100   # max ME Apps to instantiate
    *.meHost*.maxRam = 32GB	    # max Ram 
    *.meHost*.maxDisk = 100TB   # max Disk Space 
    *.meHost*.maxCpuSpeed = 400000  	# max CPU
    #----------------------------------------
    *.meHost*.eNBList = "gNodeB1"  # gNBs associated to the MEC Hosts
    
    #-------REST Services:---------------
    # MEC host 2 services configurations
    *.meHost2.mecPlatform.numMecServices = 1
    *.meHost2.mecPlatform.mecService[0].typename = "LocationService"
    *.meHost2.mecPlatform.mecService[0].localAddress = "meHost2.mecPlatform"
    *.meHost2.mecPlatform.mecService[0].localPort = 10020
    
    *.meHost2.mecPlatform.serviceRegistry.localAddress = "meHost2.mecPlatform"
    *.meHost2.mecPlatform.serviceRegistry.localPort = 10021
    
    # MEC hosts associated to the MEC system
    **.mecOrchestrator.mecHostList = "meHost1, meHost2"      
    # the MECPM needs to know the MEC orchestrator
    **.meHost*.mecPlatformManager.mecOrchestrator = "mecOrchestrator"
    # List of MEC app descriptors to be onboarded during initialization
    **.mecOrchestrator.mecApplicationPackageList = "WarningAlertApp" 
    \end{lstlisting}




\begin{lstlisting}
*.natRouter.ipv4.natTable.config = xml("<config> \
                       <entry type='prerouting' \
                      packetDataFilter='*Ipv4Header and destAddress=~10.0.2.1' \
                       srcAddress='10.0.3.2' destAddress='192.168.2.2'/> \
                       <entry type='prerouting' \
                      packetDataFilter='*Ipv4Header and destAddress=~10.0.3.2' \
                       srcAddress='10.0.2.1' destAddress='192.168.3.2'/> \
                       </config>")
\end{lstlisting}

==> temptex <==
\begin{lstlisting}
{
    "appDid" : "WAMECAPP",
    "appName" : "MECWarningAlertApp",
    "appProvider" : "lte.apps.mec.warningAlert.MECWarningAlertApp",
    "virtualComputeDescriptor" :{
        "virtualDisk": 10,
        "virtualCpu" : 1500,
        "virtualMemory":10
    },
    "appServiceRequired": [{
        "ServiceDependency" :{
            "serName" : "LocationService",
            "version" : "v2",
            "serCategory": "Location"
        }
    }
    ]
}
\end{lstlisting}


\begin{lstlisting}
#------------UEWarningAlertApp---------------
*.car[*].numApps = 2

# .car[*].app[0] is the DeviceApp
*.car[*].app[0].typename = "DeviceApp"
*.car[*].app[0].localPort = 4500
*.car[*].app[0].lcmProxyAddress = "lcmProxy"
*.car[*].app[0].lcmProxyPort = 1000

*.car[*].app[1].typename = "UEWarningAlertApp"
# Device App address
*.car[*].app[1].destAddress = "car["+string(ancestorIndex(1))+"]"   
# Device App port
*.car[*].app[1].destPort = 4500   
\end{lstlisting}





\begin{lstlisting}
    ######################_MEC Hosts Side_#####################
    # available resources 
    *.meHost*.maxMEApps = 100   # max ME Apps to instantiate
    *.meHost*.maxRam = 32GB	    # max Ram 
    *.meHost*.maxDisk = 100TB   # max Disk Space 
    *.meHost*.maxCpuSpeed = 400000  	# max CPU
    #----------------------------------------
    *.meHost*.eNBList = "gNodeB1"  # gNBs associated to the MEC Hosts
    
    #-------REST Services:---------------
    # MEC host 2 services configurations
    *.meHost2.mecPlatform.numMecServices = 1
    *.meHost2.mecPlatform.mecService[0].typename = "LocationService"
    *.meHost2.mecPlatform.mecService[0].localAddress = "meHost2.mecPlatform"
    *.meHost2.mecPlatform.mecService[0].localPort = 10020
    
    *.meHost2.mecPlatform.serviceRegistry.localAddress = "meHost2.mecPlatform"
    *.meHost2.mecPlatform.serviceRegistry.localPort = 10021
    
    # MEC hosts associated to the MEC system
    **.mecOrchestrator.mecHostList = "meHost1, meHost2"      
    # the MECPM needs to know the MEC orchestrator
    **.meHost*.mecPlatformManager.mecOrchestrator = "mecOrchestrator"
    # List of MEC app descriptors to be onboarded during initialization
    **.mecOrchestrator.mecApplicationPackageList = "WarningAlertApp" 
    \end{lstlisting}




\begin{lstlisting}
*.natRouter.ipv4.natTable.config = xml("<config> \
                       <entry type='prerouting' \
                      packetDataFilter='*Ipv4Header and destAddress=~10.0.2.1' \
                       srcAddress='10.0.3.2' destAddress='192.168.2.2'/> \
                       <entry type='prerouting' \
                      packetDataFilter='*Ipv4Header and destAddress=~10.0.3.2' \
                       srcAddress='10.0.2.1' destAddress='192.168.3.2'/> \
                       </config>")
\end{lstlisting}
